Spatio-Temporal Turbulence Mitigation: A Translational Perspective

Recovering images distorted by atmospheric turbulence is a challenging inverse problem due to the stochastic nature of turbulence. Although numerous turbulence mitigation (TM) algorithms have been proposed, their efficiency and generalization to real-world dynamic scenarios remain severely limited. Building upon the intuitions of classical TM algorithms, we present the Deep Atmospheric TUrbulence Mitigation network (DATUM). DATUM aims to overcome major challenges when transitioning from classical to deep learning approaches. By carefully integrating the merits of classical multi-frame TM methods into a deep network structure, we demonstrate that DATUM can efficiently perform long-range temporal aggregation using a recurrent fashion, while deformable attention and temporal-channel attention seamlessly facilitate pixel registration and lucky imaging. With additional supervision, tilt and blur degradation can be jointly mitigated. These inductive biases empower DATUM to significantly outperform existing methods while delivering a tenfold increase in processing speed. A large-scale training dataset, ATSyn, is presented as a co-invention to enable generalization in real turbulence. Our code and datasets are available at https://xg416.github.io/DATUM.

==> my_sec/1_introduction.tex <==
\section{Introduction}
\label{sec:intro}

%% general
%The inverse problem of 
Atmospheric turbulence is a dominant image degradation for long-range imaging systems. Reconstructing images distorted by atmospheric turbulence is an important task for many civilian and military applications.
%Since atmospheric turbulence is stochastic in nature, the point spread functions (PSFs) in the degradation process are the combination of content-invariant random pixel displacement (i.e., tilt) and blur.
The degradation process can be considered a combination of content-invariant random pixel displacement (i.e., tilt) and random blur.
Until recently, reconstruction algorithms have often been in the form of model-based solutions, often relying on modalities such as pixel registration and deblurring.
%Image restoration from turbulence-distorted images has been studied for decades. However, because of the difficulty of collecting real-world datasets, conventional algorithms in the pre-deep-learning era are model-based, typically relying on pixel registration and deblurring approaches. 
Although there have been many important insights into the problem, e.g., lucky imaging, they are primarily limited to static scenes with slow processing speed. 

%% Classical algorithms - insightful ideas, tightly connected to turbulence properties, but slow and hard to handle dynamic scenes.


\begin{figure}[t]
  \centering
   \includegraphics[width=\linewidth]{pics/performance.png}
   \caption{Benchmarking video restoration models for turbulence mitigation on our ATSyn-dynamic dataset. The circles in orange are other video-based TM networks, and the circles in blue are representative video deblurring and general restoration networks. The proposed Deep Atmospheric TUrbulence Mitigation network (DATUM) is state-of-the-art while highly efficient.}
   \label{fig:overall_model}
\end{figure}

%% deep learning - mostly are single frame, highly ill-posed, some multiple frame-based methods, lack of insight like conventional methods, lack of analysis of turbulence property. Common problem: 1. generalization 2. cumbersome.

With the development of physics-grounded data synthesis methods \cite{Milanfar_2013_a, Lau_2019_a, Chak_2021_a, fraser1999atmospheric, Vorontsov_2001_a, Frakes_2001_a}, data-driven algorithms have been developed in the past two years. Most existing deep learning methods focus on single-frame problems \cite{Lau_2021_a, Rai_2022_a, mei2023ltt, nair2023ddpm, Yasarla_2022_a, Nair_2021_a, Lau_2021_b, Jaiswal_2023_ICCV, Mao_2022_a}. Since the degradation is highly ill-posed, the performance of these algorithms is naturally limited, especially when 
%they attempt to generalize from the training set 
attempting to generalize to real data. On the other hand, multi-frame turbulence mitigation networks \cite{Jin_2021_a, Zhang_2022_a, Anantrasirichai_2022_a} have shown greater potential for generalization across a broader spectrum of real-world test scenarios. However, these networks are adapted from generic video restoration methods and do not reflect the insights developed by traditional methods; few turbulence-specific properties are incorporated as inductive biases into their methods. 

%. Few turbulence-specific properties are incorporated as inductive biases into their methods. 

For deep learning methods to work on real-world scenarios, two common factors hinder the application of current turbulence mitigation methods: (1) the complexity of current data-driven methods is usually high, which impedes the practical deployment of these algorithms, and (2) the data synthesis models are suboptimal, either too slow to produce large-scale and diverse datasets or not accurate enough to represent the real-world turbulence profiles, restricting the generalization capability of the model trained on the data.

%% deep learning - ours: a network that brings together the merits of conventional multi-frame turbulence mitigation methods, fast and effective, better generalization.
To overcome these pressing issues, we propose the Deep Atmospheric TUrbulence Mitigation (DATUM) network and the ATSyn dataset. We offer three contributions:
\begin{itemize}
    \item DATUM is the first deep-learning video restoration method customized for turbulence mitigation based on classical insights. By carefully integrating the merits of classical multi-frame TM methods, we propose feature-reference registration, temporal fusion, and the decoupling of pixel rectification and deblurring as effective inductive biases in the multi-frame TM challenge.
    
    \item DATUM is the first recurrent model for turbulence restoration. It is significantly more lightweight and efficient than the prior multi-frame TM methods. On both synthetic and real data, DATUM consistently surpasses the SOTA methods while being $10 \times$ faster.

    \item Through the integration of numerous theoretical and practical improvements in physics modeling over the Zernike-based simulators, we further propose an extensive, real-world inspired dataset ATSyn. Experiments on real-world data show that models trained on ATSyn significantly generalize better than those trained on alternative ones.
% training set consists of turbulence profiles including different $C_n^2$, path length, field of view, and camera parameters. Since these parameters are estimated from real-world data, the
\end{itemize}



==> my_sec/3_our_work.tex <==
\section{Proposed method}
% In this section, we introduce the Deep Atmospheric TUrbulence Mitigation (DATUM) network and the accompanied ATSyn Dataset. Before we discuss the details of the network, we first discuss how atmospheric turbulence is handled in the classic methods. 

\subsection{Insights from Classical Methods}
Image degradation by atmospheric turbulence can be roughly described by a compositional operation of the blur $\mathcal{B}$ and the tilt $\mathcal{T}$ via the relationship $\mathbf{I} = [\mathcal{B} \circ \mathcal{T}](\mathbf{J}) + \mathbf{n}$, where $\mathbf{J}$ is the clean image, $\mathbf{I}$ is the distorted image, and $\mathbf{n}$ is the noise term. Traditional algorithms handle turbulence in three steps, as illustrated in Fig. \ref{fig: network}:
\begin{itemize}
% \itemsep\setlength{0ex}
\item \textbf{Frame-to-reference registration} \cite{Milanfar_2013_a}, where a reference frame is constructed from the observed images and all images are registered with respect to the reference using optical flow. In strong turbulence or dynamic scenes, constructing a reference is often difficult.
\item \textbf{Lucky image fusion} \cite{joshi_2010_a, Anantrasirichai_2013_a}, where a ``lucky'' image is constructed by collecting the sharpest and most consistent patches from the inputs. However, if turbulence is strong, identifying lucky patches can be difficult.
\item \textbf{Blind deconvolution} \cite{Mao_2020_a}, where a final blind deconvolution algorithm is employed to sharpen the lucky image. The success and failure of this step depend heavily on how spatially uniform the blur in the lucky image is. Oftentimes, since the blur is spatially varying, the performance of blind deconvolution is limited.
\end{itemize}
While each step is important each has its limitations, motivating us to develop end-to-end trained networks to approximate these functions. Empowered by training on our physical-grounded dataset, our network enjoys the inductive biases of those insights while avoiding their limitations.


% This section introduces the proposed method, including the Deep Atmospheric TUrbulence Mitigation (DATUM) network and the Atmospheric Turbulence Synthesis (ATSyn) dataset. Before introducing the details of our method, we first model the turbulence degradation to an image $\boldsymbol{J}$ \cite{Chan_2022_a}:
% \begin{equation}
%     \boldsymbol{I} = [\blur \circ \tilt] (\boldsymbol{J})+\boldsymbol{n}.
%     \label{eq: forward_process}
% \end{equation}
% where $[\blur \circ \tilt]$ is the ``tilt-then-blur'' turbulence operator with $\blur$ and $\tilt$ as blur and tilt, respectively. $\boldsymbol{J}\in \mathbb{R}^{H\times W}$ is the clean input image, $\boldsymbol{I}\in \mathbb{R}^{H\times W}$ is the captured image degraded by turbulence, and $\boldsymbol{n}\in \mathbb{R}^{H\times W}$ is Gaussian noise. A fundamental property of physics embodied in \eref{eq: forward_process} is that the degradation is \emph{spatially and temporally varying}~\cite{chan2023computational}.
% %A fundamental property of \eref{eq: forward_process} is that the degradation is \emph{spatially and temporally varying} \cite{chan2023computational}.


\subsection{DATUM network}
\label{sec: network}

\subsubsection{Overview}
The block diagram of the DATUM network is depicted in Fig. \ref{fig: network}. We first summarize these three components and describe them in detail in the next subsections.

\textbf{Feature-to-reference registration}. This component is analogous to the classical frame-to-reference registration. For each input frame $I_t$ at time $t$, we first extract three levels of features $f_t^{\{1,2,3\}}$. We propose the Deformable Attention Alignment Block (DAAB) to register the high-level feature $f_t^3$ to a previously hidden reference map $r'_{t-1}$. We also propose the Gated Reference Update Module (GRUM) updates this reference feature recurrently, which is inspired by the gated recurrent unit \cite{CGRU, chung2014empirical} and illustrated in Fig. \ref{fig: network}.

\textbf{Temporal fusion}. This component is analogous to the classical lucky fusion step. The registered feature $f_t$, together with $r'_{t-1}$ and $f_t^3$, are fused by a new Deep Integration Module (DIM). DIM consists of a series of Residual Dense Blocks (RDB) \cite{zhang2018residual} and is used to produce the forward embedding $e_t^{fw}$. Since $e_t^{fw}$ is a deep feature, it is presumed to be free of tilt and is thus utilized for updating the reference feature for the subsequent frame. After the bidirectional recurrent process, we perform a temporal fusion of $e_t^{fw}$ by augmenting it with the backward embedding $e_t^{bw}$ and bidirectional embeddings from neighboring frames. We propose the Multi-head Temporal-Channel Self-Attention (MTCSA) module for this purpose.

\textbf{Post processing}. In the final stage, the temporally fused features are decoded to form the turbulence-free image. This decoding involves a twin of decoders. The first predicts a reverse tilt map that rectifies the shallow features, and the second subsequently reconstructs the clean image.


% \subsubsection{Overview}
% The DATUM network, depicted in Fig. \ref{fig: network}, is inspired by traditional turbulence mitigation (TM) methods and encompasses three main stages: feature-to-reference registration, temporal fusion, and post-processing. 

% \textbf{Feature-to-reference registration}. For each input frame $I_t$ at time $t$, we first extract three levels of features $f_t^{\{1,2,3\}}$. The Deformable Attention Alignment Block (DAAB) then registers the high-level feature $f_t^3$ to a previously hidden reference map $r'_{t-1}$. Subsequently, the Gated Reference Update Module (GRUM) updates this reference feature recurrently, as illustrated in Fig. \ref{fig: network}.

% \textbf{Temporal fusion}. The registered feature $f_t$, together with $r'_{t-1}$ and $f_t^3$, are fused by the Deep Integration Module (DIM). DIM consists of a series of Residual Dense Blocks (RDB) \cite{zhang2018residual} and is used to produce the forward embedding $e_t^{fw}$. Since $e_t^{fw}$ is a deep feature, it is presumed to be free of tilt and is thus utilized for updating the reference feature for the subsequent frame.

% After the bidirectional recurrent process, we perform a temporal fusion of $e_t^{fw}$ by augmenting it with the backward embedding $e_t^{bw}$ and bidirectional embeddings from neighboring frames. Unlike classical methods that employ region-based selection and weighting for fusion (often referred to as ``lucky fusion''), the DATUM network adopts a spatially independent temporal selection and weighting at the feature level for better adaptability. This is accomplished through the Multi-head Temporal-Channel Self-Attention (MTCSA) module. 

% \textbf{Post processing}. In the final stage, the temporally fused features are decoded to form the turbulence-free image. This decoding involves a twin of decoders. The first predicts a reverse tilt map that rectifies the shallow features, and the second subsequently reconstructs the clean image.

\subsubsection{Components}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width = \linewidth]{pics/DAAB.png}
%     \caption{Scheme of Deformable Attention Alignment Block}
%     \label{fig: synthesis}
% \end{figure}
\noindent \textbf{Feature registration via Deformable Attention Alignment Block (DAAB).}
In classical methods, a crucial stage for turbulence mitigation is registering the input frames to the tilt-free reference frame. This reference frame is usually obtained by temporal averaging or using variants of principle component analysis. However, these methods may not be applicable to dynamic videos. Since learning-based video TM is possible \cite{Zhang_2022_a, Jin_2021_a}, the deep feature of a video TM network can be considered tilt-mitigated to work as the reference feature for the next input feature. This section explains our method to use deformable attention to facilitate feature registration in our DATUM network.

The computations in the DDAB are summarized in Algorithm 1, where $\warp(A;B)$ denotes warping $A$ by deformation field $B$, $\phi(A;p)$ denotes sampling $A$ by positions $p$. $W_K$, $W_V$, $W_Q$, and $W$ are linear projections on the channel dimension, and $\sigma$ denotes the SoftMax. The optical flow at line 3 is estimated with the SPyNet \cite{Ranjan_2017_a}, and lines 6-11 are inspired by the guided deformation attention (GDA) \cite{liang2022rvrt}.

% We first find a rough deformation field $\hat{O}_{t}^{f\rightarrow r}$ between the input feature of the current frame $f_t^3$ and the reference feature from the last frame $r'_{t-1}$. $\hat{O}_{t}^{f\rightarrow r}$ can be estimated from the optical flow estimation $O_{t\rightarrow t-1}^{f}$ between frames $I_{t}$ and $I_{t-1}$ and the deformation field $O_{t-1}^{f\rightarrow r}$ by
% \begin{equation}
%     \hat{O}_{t}^{f\rightarrow r} = O_{t-1}^{f\rightarrow r} + \warp(O_{t\rightarrow t-1}^{f}; O_{t-1}^{f\rightarrow r}). 
% \end{equation}
% where $\warp(A;B)$ denotes warping $A$ by deformation field $B$. The input feature is then registered to the reference frame by the multi-group multi-head deformation attention module proposed in \cite{liang2022rvrt}. In this module, $\hat{O}_{t}^{f\rightarrow r}$ functions as the foundational offset, which is further refined by residual offsets $\{\Delta o_{t}^{g}\}$ where $g$ is the index of the group. $\{\Delta o_{t}^{g}\}$ are predicted from the pre-aligned feature $\hat{f}_{t} = \warp(\hat{O}_{t}^{f\rightarrow r}, f_{t}^{3})$ and reference $r'_{t-1}$ by a Residual Dense Block (RDB). The final offset for the $g \text{-th}$ group is computed by $o^{g}_{t} = \hat{O}_{t}^{f\rightarrow r} + \Delta o_{t}^{g}$, and we can update the final alignment flow $O_{t}^{f\rightarrow r}$ by the mean of $\{o^{g}_{t}\}$.

% The input feature $f_{t}^{3}$ is projected by $W_{K}$ and $W_{V}$ to form the key $K$ and value $V$, the reference $r'_{t-1}$ is projected by $W_{Q}$ form the query $Q$. The aligned feature $\hat{f}_t$ from the deformable attention is drawn by \cite{Xia_2022_CVPR}:
% \begin{equation}
% \begin{aligned}
%     K &= \phi(f_{t}^{3}W_{K}; o_{t}) \quad V = \phi(f_{t}^{3}W_{V}; o_{t})  \\
%     Q &= r'_{t-1}W_{Q}  \quad\quad  \hat{f}_t = \sigma(QK^T / \sqrt{C}) V &
% \end{aligned}
% \end{equation}
% where $\phi(x;o_{t})$ denotes sampling $x$ on the feature grid with offset $o_{t}$, $\sigma$ denotes the SoftMax function and $C$ is the channel dimension of $K$, $V$ and $Q$. Finally, the aligned feature $\hat{f}_t$ and reference $r'_{t-1}$ are fused by a feedforward network (FFN) to generate the updated reference $r_t$.

\begin{algorithm}
\caption{Deformation Attention Alignment Block}
\begin{algorithmic}[1]
\State \textbf{Input:} Current frame feature $f_t^3$, reference feature $r'_{t-1}$ and alignment flow from last frame $O_{t-1}^{f\rightarrow r}$, two downsampled frames $I_t$ and $I_{t-1}$
\State \textbf{Output:} Updated feature $f_t$ and flow $O_{t}^{f\rightarrow r}$

\Statex \Comment{Estimate rough deformation field $\hat{O}_{t}^{f\rightarrow r}$ that register feature $f_t^3$ to reference $r'_{t-1}$}

\State Estimate the optical flow $O_{t\rightarrow t-1}^{f}$ from $I_t$ and $I_{t-1}$.

\State $\hat{O}_{t}^{f\rightarrow r} \leftarrow O_{t-1}^{f\rightarrow r} + \warp(O_{t\rightarrow t-1}^{f}; O_{t-1}^{f\rightarrow r})$
\State Pre-align $\hat{f}_{t} \leftarrow \warp(\hat{O}_{t}^{f\rightarrow r}, f_{t}^{3})$
\LineComment{Register input feature to reference frame using multi-group multi-head deformation attention}

\ForAll{group $g$}
     \Statex \hskip\algorithmicindent $\triangleright$ Predict offsets $o_{t}^{(g)}$
    \State $\Delta o_{t}^{(g)} \leftarrow \text{RDB}(\text{Concat}(\hat{f}_{t}, r'_{t-1}, \hat{O}_{t}^{f\rightarrow r}))$
    \State $o^{(g)}_{t} \leftarrow \hat{O}_{t}^{f\rightarrow r} + \Delta o_{t}^{(g)}$
    \Statex \hskip\algorithmicindent $\triangleright$ Compute the $g\text{-th}$ aligned feature $\hat{f}_t^{(g)}$:
    \State $K^{(g)} \leftarrow \phi(f_{t}^{3}W_{K}; o^{(g)}_{t})$, $V^{(g)} \leftarrow \phi(f_{t}^{3}W_{V}; o^{(g)}_{t})$
    \State $Q \leftarrow r'_{t-1}W_{Q}$, $\hat{f}^{(g)}_t \leftarrow \sigma(QK^{(g)T} / \sqrt{C}) V^{(g)}$
\EndFor

\State Fuse all groups $f_t \leftarrow \text{Concat}(\{\hat{f}^{(g)}_t\})W$
\State Update final alignment flow $O_{t}^{f\rightarrow r}$ by mean of $\{o^{(g)}_{t}\}$
\State Output $f_t \leftarrow f_t + \text{FeedForward}(f_t)$
\end{algorithmic}
\end{algorithm}


\noindent \textbf{Temporal fusion via Multi-head Temporal Channel Self-Attention (MTCSA).}
After feature registration and deep integration, we propose to augment the embedding with contra-directional information, which is essential to ensure consistent restoration quality across various frames. In addition, like classical methods, a spatially adaptive fusion with adjacent frames is advantageous. We propose the Multi-head Temporal-Channel Self-Attention (MTCSA), as illustrated in Fig. \ref{fig: network}. The MTCSA begins by concatenating channels from multiple frames, followed by a $1 \times 1$ convolution to shrink the channel dimension. Separable convolution is used to construct the spatially varying query, key, and value on the temporal and channel dimensions, and the dynamic fusion is facilitated by self-attention. Finally, a residual connection is used to stabilize training. Considering the quadratic complexity of MTCSA relative to window size, this size is kept moderate. Additionally, we integrate a hard-coded positional embedding wherein features from the focal frame are positioned at the end. This strategy is essential for boundary frames with disproportionate neighboring frames on either side.

\noindent \textbf{Twin decoder and loss function}
 Given the refined feature embedding from the MTCSA, we also developed a twin decoder to progressively remove the tilt and blur, as shown in Fig. \ref{fig: network}. The decoder uses transposed convolution for upsampling and channel attention blocks (CAB) \cite{woo2018cbam} for decoding. Before decoding in higher levels, the deep features are concatenated with the shallow features to facilitate the residual connection like a typical UNet \cite{ronneberger2015u}. Since the deep and shallow features are misaligned by the random tilt $\calL$, we propose to first rectify the shallow features by the estimated inverse tilt field $\hat{\calT}^{-1}$ estimated in the first stage. The tilt-rectification is optimized by reducing the loss:
\begin{equation}
\label{eq:loss_tilt}
    \calL_{\text{tilt}} = \calL_{\text{char}}(\boldsymbol{I}_{\text{GT}}, \warp(\boldsymbol{I}_{\text{tilt}}; \hat{\calT}^{-1}))
\end{equation}
Where $\calL_{\text{char}}$ denotes the Charbonnier loss \cite{charbonnier}, $\boldsymbol{I}_{\text{GT}}$ is the input frame and $\boldsymbol{I}_{\text{tilt}}$ is the tilt-only frame that can be produced without additional cost by our data synthesis method. In the second stage, the rectified shallow features are jointly decoded with the deep features to generate the final reconstruction $\hat{\boldsymbol{I}}$. The overall loss function is computed by:
\begin{equation}
    \calL = \alpha_1 \calL_{\text{tilt}} + \alpha_2 \calL_{\text{char}}(\boldsymbol{I}_{\text{GT}}, \hat{\boldsymbol{I}})
\end{equation}
where weights $\alpha_1$ and $\alpha_2$ are empirically set to 0.2 and 0.8.

\subsection{ATSyn dataset}
\subsubsection{Physics-based data synthesis}
\label{sec: data_synthesis}

\begin{figure}
    \centering
    \includegraphics[width = 0.9\linewidth]{pics/synthesis.png}
    \vspace{-0.5em}
    \caption{Scheme of our data synthesis method.}
    \label{fig: synthesis}
\end{figure}

As introduced previously, the ground truth image $\boldsymbol{J}$ is first geometrically distorted and then blurred to produce the degraded image $\boldsymbol{I}$ in our synthesis method. Data synthesis for the turbulence effect essentially requires a physics-grounded representation of $\blur$ and $\tilt$. We adopted the Zernike-based turbulence simulator \cite{Chimitt_2020_a, chimitt2022real} and improved it with non-trivial modifications. Fig. \ref{fig: synthesis} presents the scheme of our implementation. The $\blur$ and $\tilt$ is generated from the phase distortion represented by Zernike polynomials $\{\mZ_i\}$ \cite{Noll_1976_a} as the basis, with corresponding coefficients $\va_{i}$ where $i$ ranging from 1 to 36. Among all 36 coefficients, $i=1$ denotes the current component, $i={2,3}$ controls the $\tilt$ by a constant scale, and the rest high order Zernike coefficients contribute to the blur effect.

 The phase distortion can be assumed as a wide sense stationary (WSS) random field \cite{chimitt2022real}. Hence, it can be sampled with Fast Fourier Transform (FFT) from white Gaussian noise and the autocorrelation map. Transforming the phase distortion to the spatial domain point spread functions (PSF) can be achieved by the Phase-to-Space (P2S) transform, which transforms the sampled Zernike coefficients to spatial coefficients $\boldsymbol{\beta}$, assuming the PSFs can be represented by a low-rank approximation of 100 basis $\boldsymbol{\psi}$ and corresponding $\boldsymbol{\beta}$. The overall degradation in the spatial domain is implemented by 
\begin{equation}
    \boldsymbol{I} = \sum_{k=1}^{100}\boldsymbol{\psi}_k \circledast (\boldsymbol{\beta}_{k} \cdot \warp(\boldsymbol{J}; \tilt)) + \boldsymbol{n},
    \label{eq: p2s_psf_basis}
\end{equation}
where $\circledast$ denotes the depth-wise convolution. Although subtle, this fundamentally generates more reliable degradation than the simulator in \cite{Zhang_2022_a}, as elaborated in \cite{Chimitt_2023_b}. Except for this, our correlation kernels are more precise by incorporating the continuous $C_{n}^{2}$ path technique \cite{Chimitt_2023_a}.


\subsubsection{Guideline of implementation}

With the proposed simulator, we created the ATSyn dataset to match various real-world turbulence conditions and benchmark deep neural networks for turbulence mitigation. This dataset is segmented into two distinct subsets based on scene type: the \emph{ATSyn-dynamic} and \emph{ATSyn-static}. The dynamic sequences contain camera or object motion, whereas the static sequences are each associated with only one underlying clean image. We adopted parameters including focal length, F-number, distance, wavelength, scene size, and sensor resolution to control the simulation. In comparison with the synthetic dataset introduced in \cite{Zhang_2022_a}, which utilized the $D/r_0$ \cite{Fried_1965_a} and empirically chosen blur kernel size, our dataset's parameter space more closely aligns with actual camera settings, making it more representative. 
% Since the available real-world static sequences from \cite{UG2, Gilles_2017_a} have narrower FOV than the dynamic scene videos from \cite{Anantrasirichai_2022_a, Jin_2021_a}, they have visually stronger turbulence degradation. The ATSyn also reflects this difference by setting a narrower field of view, hence a larger blur kernel and tilt magnitude to our static sequences. 

ATSyn-dynamic contains 4,350 training and 1,097 validation instances synthesized from \cite{Safdarnejad_2015_a, Jin_2021_a}, and ATSyn-static contains 2,000 and 1,000 instances synthesized from the Places dataset \cite{zhou2017places} for training and validation, respectively. Those instances have varying numbers of frames, each with a distinct turbulence parameter set. Besides ground truth and fully degraded videos, ATSyn further provides associated $\boldsymbol{\mathcal{T}}$-only videos to facilitate the training of $\calL_{\text{tilt}}$ in Eq. \ref{eq:loss_tilt}. We categorize the turbulence parameters by three levels: \emph{weak}, \emph{medium}, and \emph{strong}. The range of turbulence parameters is determined by matching with a large-scale, long-range video dataset \cite{cornett2023expanding} and other real-world videos, with more details in the supplementary document.

% Besides our ATSyn, we also used \cite{Zhang_2022_a}'s synthetic dataset for a preliminary study. There are 3500 instances for training and 1184 for validation in this dataset synthesized from the same source videos as ATSyn. We tested the generalization of our model on real-world images from \cite{Anantrasirichai_2022_a, Jin_2021_a, Gilles_2017_a, UG2}. Among them, videos in \cite{Anantrasirichai_2022_a, Jin_2021_a} are mostly dynamic, \cite{Gilles_2017_a} and \cite{UG2} provide static scene image sequences to benchmark the turbulence mitigation algorithms, the OTIS dataset \cite{Gilles_2017_a} has 16 pattern image sequences in various turbulence conditions and \cite{UG2} provides a turbulence-text dataset. The turbulence-text dataset contains 100 sequences, each a static scene of degraded text patterns at 300 meters and further. In the place of ground truth, which is impossible in real-world turbulence, this benchmark uses the accuracy score of pre-trained text recognition models CRNN \cite{shi2016end}, DAN \cite{wang2020decoupled}, and ASTER \cite{shi2018aster} as its metrics, with a better restoration method offering better recognition performance.


==> my_sec/4_experiments.tex <==
\section{Experiments}

\begin{table*}
\centering
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{c|cccccccc}
\hline
Methods & TurbNet \cite{Mao_2022_a} & TSRWGAN \cite{Jin_2021_a} & VRT \cite{liang2022vrt}  & TMT \cite{Zhang_2022_a} & RNN-MBP \cite{zhu2022deep} & ESTRNN \cite{zhong2022real} & RVRT \cite{liang2022rvrt} & DATUM [ours]  \\
\hline
PSNR &  24.2229 & 26.3262 & 27.6114 & 27.7419 & 27.7152 & 27.3469 &  27.8512 & \textbf{28.5875} \\
$\text{SSIM}_{\text{CW}}$ &  0.8230 & 0.8596 & 0.8691 & 0.8741 & 0.8730 & 0.8617 & 0.8788 & \textbf{0.8803}  \\
\hline
\end{tabular}
}
\vspace{-0.5em}
\caption{Preliminary study: evaluate on TMT's synthetic dynamic scene data \cite{Zhang_2022_a}. $\text{SSIM}_{\text{CW}}$ denotes Complex Wavelet SSIM.}
\label{table:pre}
\end{table*}

\begin{table*}
\centering
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{l|cccccccc|cc}
\toprule[0.8pt]
    Turbulence Level & \multicolumn{2}{c}{Weak} & \multicolumn{2}{c}{Medium} & \multicolumn{2}{c}{Strong}  & \multicolumn{2}{c|}{Overall} & \multicolumn{2}{c}{Cost}  \\
    \hline
    %\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}  \cmidrule(lr){8-9}  \cmidrule(lr){10-12} 
Methods & PSNR & $\text{SSIM}_{\text{CW}}$ & PSNR & $\text{SSIM}_{\text{CW}}$ & PSNR & $\text{SSIM}_{\text{CW}}$ & PSNR & $\text{SSIM}_{\text{CW}}$ & Size  & FPS \\
\hline
TSRWGAN \cite{Jin_2021_a} & 27.0844 & 0.8575 & 26.7046 & 0.8514 & 25.4230 & 0.8372 &  26.4541 & 0.8493 & 46.28 & 0.87 \\
TMT \cite{Zhang_2022_a} & 29.1183 & 0.8836  & 28.5050 & 0.8791  & 26.9744 & 0.8552  & 28.2665 & 0.8734  & 26.04 &  0.80\\
VRT \cite{liang2022vrt} & 28.8453 &  0.8797 & 28.2628 & 0.8769  & 26.7492 & 0.8506  & 28.0179 &  0.8699 & 18.32 & 0.17\\
RNN-MBP \cite{zhu2022deep} & 27.9243 &  0.8699  & 27.4742 & 0.8642 & 26.0812 & 0.8495 & 27.2161 & 0.8618 & 14.16 &  1.14 \\
ESTRNN \cite{zhong2022real} & 28.9805 & 0.8750  & 28.3338 & 0.8697   & 26.8897 & 0.8463  & 28.1347 & 0.8645 & 2.468 & 27.65\\
RVRT \cite{liang2022rvrt} & 29.6080 &  0.8845 & 28.9605 & 0.8806 & 27.5344 &  0.8595 & 28.7672 & 0.8756 & 13.50 & 2.43 \\
% \rowcolor{Gray}DATUM-s [ours] & 29.5958 & 0.8809 & 28.9869 & 0.8762 & 27.5456 & 0.8550 & 28.7743 & 0.8714 & 2.538 & 22.48 \\
\rowcolor{Gray}DATUM [ours] & \textbf{30.2058} & \textbf{0.8857} & \textbf{29.6203} & \textbf{0.8829} & \textbf{28.2550} & \textbf{0.8640} & \textbf{29.4222} & \textbf{0.8781}  & 5.754 & 9.17 \\
\bottomrule[0.8pt]
\end{tabular}
}
\vspace{-0.5em}
\caption{Performance comparison on the ATSyn-dynamic set, we list the image quality scores on different turbulence levels and frame-wise resource consumption (measured with $960\! \times \! 540$ frame sequences on RTX 2080 Ti).}
\label{table:dynamic}
\end{table*}

\subsection{Training setting}
This section describes how we trained our DATUM and other models. Except for turbulence mitigation networks \cite{Jin_2021_a, Zhang_2022_a, Mao_2022_a}, we also benchmarked several representative video restoration \cite{liang2022vrt, liang2022rvrt} and deblurring networks \cite{zhong2022real,zhu2022deep} for a more thorough comparison.

To train the proposed model, we used the Adam optimizer \cite{kingma2014adam} with the Cosine Annealing learning rate schedule \cite{loshchilov2016sgdr}. The initial learning rate is $2\times 10^{-4}$, and batch size is 8. All dynamic scene TM networks in this experiment are trained end-to-end from scratch for 800K iterations. To get their static-scene variant, we fine-tuned them on the static-scene modality with half the initial learning rate and 400K iterations. We clip the gradient if the L2 norm exceeds 20 to prevent gradient explosion during inference.

We trained the ESTRNN \cite{zhong2022real}, RNN-MBP \cite{zhu2022deep}, and RVRT \cite{zhong2022real} with the same configuration as DATUM. The number of input frames of DATUM and ESTRNN during training is set to 30 for ATSyn-dynamic and 36 for ATSyn-static. Since RNN-MBP and RVRT require much more resources to train, the number of input frames is set to 16. Because TSRWGAN \cite{Jin_2021_a}, TMT \cite{Zhang_2022_a}, and TurbNet \cite{Mao_2022_a} are all designed for turbulence mitigation, we trained them following the original paper and public code. 

\subsection{Comparison on dynamic scene modality}
We first trained and evaluated all networks for comparison on a previous Zernike-based synthetic dataset \cite{Zhang_2022_a} for preliminary study. We choose PSNR and Complex Wavelet Structure Similarity \cite{sampat2009complex} (CW-SSIM) as the criterion in this paper, and the reason for selecting CW-SSIM rather than SSIM is provided in the supplementary document. The result in Table \ref{table:pre} shows our DATUM outperforms the previous state-of-the-art TMT \cite{Zhang_2022_a} with $5\times$ fewer parameters and over $10 \times$ faster inference speed. We also benchmark a representative single-frame TM network \cite{Mao_2022_a} to demonstrate the superiority of multi-frame TM methods. Next, we present extensive results from the ATSyn-dynamic dataset in Table \ref{table:dynamic}. Our model outperforms all other networks by a significant margin, while it is the second smallest network among all models and the most efficient network among all existing turbulence mitigation networks. 

% Although RVRT \cite{liang2022rvrt} is the SOTA network on general video restoration tasks, the performance on turbulence mitigation is not ideal. Like many other advanced video restoration networks, they heavily rely on optical flow estimation. However, due to the random pixel jittering under atmospheric turbulence, optical flow estimators always fail or generate a random field, leading to suboptimal results for those networks.

\subsection{Comparison on static scene modality}

When training on the ATSyn-static, the loss is computed between the single ground truth and all output frames. For testing, we instead calculate the average score of the central four frames in the entire output sequence (for single-directional models, we use the last 4). We evaluated the performance on the ATSyn-static and the turbulence text dataset \cite{UG2}, and the result is shown in Table \ref{table:static}. The turbulence text dataset contains 100 sequences of text images, each a static scene of degraded text pattern captured at 300 meters or farther. Real-world turbulence videos do not have ground truth, while \cite{UG2} uses the accuracy score of pre-trained text recognition models CRNN \cite{shi2016end}, DAN \cite{wang2020decoupled}, and ASTER \cite{shi2018aster} as metrics, where a better turbulence mitigation offers better recognition performances. Our model is trained on a wide range of turbulence conditions and generic data, without specific augmentation tricks, yet performs on par with the best systems in the $\text{UG2+}$ turbulence challenge \cite{UG2}. Our model outperforms other networks trained on the ATSyn-static dataset by an even larger margin.
%Add results of the coded-target? 

\begin{table}
\centering
\small
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}
\resizebox{0.47\textwidth}{!}{
\begin{tabular}{lccc}
\toprule[1pt]
Benchmark & \multicolumn{2}{c}{ATSyn-static} & Turb-Text ($\%$) \\
 \cmidrule(r){1-1} \cmidrule(r){2-3} \cmidrule(r){4-4} 
 Methods & PSNR & $\text{SSIM}_{\text{CW}}$ & CRNN/DAN/ASTER \\
\midrule
TSRWGAN \cite{Jin_2021_a} & 23.16 & 0.8407 & 60.30 / 73.90 / 74.40 \\ 
TMT \cite{Zhang_2022_a} & 24.51 & 0.8716 & 80.90 / 87.25 / 88.55 \\
VRT \cite{liang2022vrt} & 24.27 & 0.8641 & 76.30 / 84.45 / 83.60 \\
RNN-MBP \cite{zhu2022deep} & 24.64 & 0.8775 & 51.35 / 65.00 / 64.30\\
ESTRNN \cite{zhong2022real} & 26.23 & 0.9017 & 87.10 / 97.80 / 96.95 \\
RVRT \cite{liang2022rvrt} & 25.71 & 0.8876 & 86.40 / 89.00 / 89.20 \\
\rowcolor{Gray} DATUM [ours]  & \textbf{26.76} & \textbf{0.9102} & \textbf{93.55 / 97.95 / 97.25} \\%26.61
\bottomrule[1pt]
\end{tabular}
}
\vspace{-0.5em}
\caption{Static scene modality. CRNN/DAN/ASTER are the text recognition rates of these three models from the restored images.}
\label{table:static}
\vspace{-0.5em}
\end{table}

\subsection{Ablation study}
Our ablation study examines key elements that introduce effective inductive biases of our model, including the use of additional frames, recurrent reference updating, feature-reference registration, and multi-frame embedding fusion. 


\noindent \textbf{Influence of the number of input frames.}
The number of input frames for both training and inference matters for recurrent-based networks, especially in turbulence mitigation. Since turbulence degradation is caused by zero-mean stochastic phase distortion, the more frames the network can perceive, the better the non-distortion state it can evaluate. This is particularly valid for static scene sequences, where the pixel-level turbulence statistics are much easier to track and analyze through time.

We trained two models with 12-frame and 24-frame inputs and presented their respective performance during inference in Fig. \ref{fig: temporal_len}. This figure shows in the temporal range of our experimental setting, a positive correlation between the performance and the number of input frames always exists, especially on the static scene modality where an over 1 dB boost can be obtained with more frames. This phenomenon suggests one of the success factors for turbulence mitigation is the capability of fusing more frames, similar to the video super-resolution problem \cite{chan2022investigating}. 
%The same phenomenon keeps in real-world text sequences. When using 30 frames, the recognition rate is $94.1\%$, and when using all 100 frames, the accuracy boosts to $97.5\%$, suggesting our model scales well on the temporal dimension.

\begin{figure}
    \centering
    \footnotesize
    \begin{tabular}{cc}
        \includegraphics[width = 0.45\linewidth]{pics/test_dyn_2.pdf} &
        \includegraphics[width = 0.45\linewidth]{pics/test_stat_2.pdf} \\
        (a) On ATSyn-dynamic &  (b) On ATSyn-static
    \end{tabular}
    \vspace{-0.5em}
    \caption{Influence of the number of input frames.}
    \vspace{-1em}
    \label{fig: temporal_len}
\end{figure}

\noindent \textbf{Influence of DAAB, MTCSA, GRUM, and twin decoder.}
The design of DAAB and MTCSA are inspired by pixel registration and lucky fusion in the conventional TM methods. Although our spatial registration and temporal fusion are implemented at the feature level, they are still effective in turbulence mitigation, as shown in Table \ref{table:ablation}.

While the MTCSA fuses embeddings from multiple frames in a sliding window manner, determining the optimal window size is crucial. If the window size is too small, the temporal fusion only relies on the implicit temporal propagation by the recurrent unit, limiting the performance; if the window size is too large, because of the quadratic complexity along the temporal dimension, the MTCSA becomes very resource-demanded, and the network becomes less flexible to deal with a small number of input frames. We investigated the temporal window size of the MTCSA module, as shown in Fig. \ref{table:ablation}, where we found that five frames meet the trade-off between performance and efficiency. 

The GRUM utilizes a gating mechanism in the recurrent network to facilitate more extended temporal dependency \cite{CGRU, chung2014empirical}. It fuses the reference feature with deeper embeddings in a more adaptive manner, which also turns out to be effective. Finally, in the post-processing stage, we compared the two-stage twin decoder with the one-stage plain decoder. We found that by incorporating additional supervision and rectifying shallow features in the decoding stage, better performance can be obtained.

\begin{table}
\centering
\resizebox{0.47\textwidth}{!}{
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}
\begin{tabular}{lccc}
\toprule[0.8pt]
Components & PSNR / SSIM & Size & GMACs \\
\midrule
\hspace{0.5em} Base (MTCSA-1f)  &  28.62 / 0.8465 & 3.912 & 261.5 \\
% 12.09 fps
\hspace{0.5em} Base (MTCSA-3f) & 28.79 / 0.8497 & 4.131 & 272.7 \\ 
$\ast$ Base (MTCSA-5f) & 28.87 / 0.8522 & 4.768  & 304.2 \\ 
\hspace{0.5em} Base (MTCSA-7f) & 28.92 / 0.8532 & 5.808 & 358.1 \\ 

+ GRUM  &  29.06 / 0.8576 & 4.894 & 317.7  \\
% 10.83 fps
+ DAAB & 29.33 / 0.8638 & 5.241 & 351.8 \\ 
% 12.76 fps
+ Twin Decoder & 29.42 / 0.8647 & 5.754 & 372.7 \\ 
\bottomrule[0.8pt]
\end{tabular}
}
\vspace{-0.5em}
\caption{Ablation study. We conducted experiments on the ATSyn-dynamic set by adding each proposed component progressively and observed a constant performance improvement.}
\label{table:ablation}
\end{table}

\begin{figure}
    \centering
    \includegraphics[width = 0.9\linewidth]{pics/TurbText.png}
    \vspace{-0.6em}
    \caption{Comparison on the real-world turbulence-text dataset. The metric is the average text recognition accuracy of CRNN, DAN, and ASTER tested on the restored images.}
    \label{fig:quant_text}
\end{figure}


\subsection{Comparison on real-world data}

\begin{figure*}[ht]
    \captionsetup[subfloat]{font=scriptsize}
    \centering
  \subfloat[Input frame]{%
      \includegraphics[width=0.14\linewidth]{pics/pg94_new/input.jpg}}
    \hfill
  \subfloat[TSRWGAN \cite{Jin_2021_a}]{%
    \includegraphics[width=0.14\linewidth]{pics/pg94_new/TSRWGAN_original.jpg}}
   \hfill
  \subfloat[TMT \cite{Zhang_2022_a}]{%
        \includegraphics[width=0.14\linewidth]{pics/pg94_new/TMT_original.jpg}}
    \hfill
  \subfloat[NDIR \cite{Li_2021_a}]{%
      \includegraphics[width=0.14\linewidth]{pics/pg94_new/NDIR.jpg}}
    \hfill
  \subfloat[TurbNet \cite{Mao_2022_a}]{%
        \includegraphics[width=0.14\linewidth]{pics/pg94_new/TurbNet.jpg}}
    \hfill
  \subfloat[AT-DDPM \cite{nair2023ddpm}]{%
      \includegraphics[width=0.14\linewidth]{pics/pg94_new/ATPPDM.jpg}}
    \hfill
  \subfloat[PiRN \cite{Jaiswal_2023_ICCV}]{%
      \includegraphics[width=0.14\linewidth]{pics/pg94_new/PiRN.jpg}}
    \hfill
    
  \subfloat[\textbf{DATUM [Ours]}]{%
      \includegraphics[width=0.14\linewidth]{pics/pg94_new/DATUM.jpg}}
    \hfill
  \subfloat[TSRWGAN* \cite{Jin_2021_a}]{%
    \includegraphics[width=0.14\linewidth]{pics/pg94_new/TSRWGAN.jpg}}
   \hfill
  \subfloat[TMT* \cite{Zhang_2022_a}]{%
        \includegraphics[width=0.14\linewidth]{pics/pg94_new/TMT_new.jpg}}
    \hfill
  \subfloat[RNN-MBP* \cite{Mao_2022_a}]{%
        \includegraphics[width=0.14\linewidth]{pics/pg94_new/MBP.jpg}}
    \hfill
  \subfloat[RVRT* \cite{liang2022rvrt}]{%
      \includegraphics[width=0.14\linewidth]{pics/pg94_new/RVRT.jpg}}
    \hfill
  \subfloat[VRT* \cite{Jin_2021_a}]{%
      \includegraphics[width=0.14\linewidth]{pics/pg94_new/VRT.jpg}}
    \hfill
  \subfloat[ESTRNN* \cite{zhong2022real}]{%
      \includegraphics[width=0.14\linewidth]{pics/pg94_new/ESTRNN.jpg}}
    \hfill

  \caption{Qualitative comparison on the turbulence-text dataset \cite{UG2}. The input frame (a) is the 49th frame of the 94th sequence in \cite{UG2}. Figures on the top row are restoration results of corresponding TM methods using their original model and checkpoints. Figures on the bottom row are TM or general restoration models (marked by *) trained on our \emph{ATSyn-static} dataset.}
  \label{fig:text} 
\end{figure*}

% \begin{table}
% \centering
% \small
% \setlength{\aboverulesep}{0pt}
% \setlength{\belowrulesep}{0pt}
% \resizebox{0.46\textwidth}{!}{
% \begin{tabular}{ccc}
% \toprule
%  Model &  Simulator in \cite{Zhang_2022_a}  &  Our simulator \\
% \midrule
% TSRWGAN & 57.75 / 71.45 / 73.10  & 60.30 / 73.90 / 74.40 \\
% TMT & 79.25 / 85.20 / 88.00  & 80.90 / 87.25 / 88.55 \\ 
% ESTRNN & 84.50 / 96.25 / 95.45   & 87.10 / 97.80 / 96.95 \\
% DATUM  & 91.95 / 96.40 / 95.75 & 93.35 / 97.85 / 97.05 \\
% \bottomrule
% \end{tabular}}
% \vspace{-0.5em}
% \caption{Comparison on the turbulence-text dataset. The metrics are recognition accuracy (\%) by text recognition models CRNN / DAN / ASTER from the restored images. \textcolor{red}{Need to be updated to include more methods and training data or potentially the coded-target data.}}
% \label{tab:text}
% \end{table}


\begin{table}
\centering
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}
\resizebox{0.46\textwidth}{!}{
\begin{tabular}{c|ccc}
\hline
 Face Retrieval  & Degraded &  Simulator in \cite{Zhang_2022_a} &  Our simulator \\ \hline
 Rank 5  & 37.75\%       &  38.83\%  &  \textbf{39.18\%}        \\
Rank 10 & 40.59\%        & 41.83\% & \textbf{42.18\%}        \\
Rank 20 & 45.29\%      &  46.40\%  & \textbf{46.70\%} \\
\hline
\end{tabular}}
\vspace{-0.5em}
\caption{Face recognition results on a subset of the BRIAR dataset.}
\vspace{-1em}
\label{tab:face}
\end{table}

In this section, we demonstrate our data's generalization capability qualitatively and quantitatively on real-world data. 

\begin{figure*}[ht]
    \captionsetup[subfloat]{font=scriptsize}
    \centering
  \subfloat[Input frame]{%
      \includegraphics[width=0.14\linewidth]{pics/face/face_input.jpg}}
    \hfill
  \subfloat[TSRWGAN \cite{Jin_2021_a}]{%
    \includegraphics[width=0.14\linewidth]{pics/face/face_TSRWGAN_ori.jpg}}
   \hfill
  \subfloat[TMT \cite{Zhang_2022_a}]{%
        \includegraphics[width=0.14\linewidth]{pics/face/face_TMT_old.jpg}}
    \hfill
  \subfloat[TurbNet \cite{Mao_2022_a}]{%
        \includegraphics[width=0.14\linewidth]{pics/face/face_Turbnet.jpg}}
    \hfill
  \subfloat[ATNet \cite{Nair_2021_a}]{%
      \includegraphics[width=0.14\linewidth]{pics/face/face_ATNet.png}}
    \hfill
  \subfloat[AT-DDPM \cite{nair2023ddpm}]{%
      \includegraphics[width=0.14\linewidth]{pics/face/face_ATDDPM.jpg}}
    \hfill
  \subfloat[PiRN-SR \cite{Jaiswal_2023_ICCV}]{%
      \includegraphics[width=0.14\linewidth]{pics/face/face_PiRN.jpg}}
    \hfill

  \subfloat[\textbf{DATUM* [Ours]}]{%
      \includegraphics[width=0.14\linewidth]{pics/face/face_DATUM.jpg}}
    \hfill
  \subfloat[TSRWGAN* \cite{Jin_2021_a}]{%
    \includegraphics[width=0.14\linewidth]{pics/face/face_TSRWGAN_.jpg}}
   \hfill
  \subfloat[TMT* \cite{Zhang_2022_a}]{%
        \includegraphics[width=0.14\linewidth]{pics/face/face_TMT_new.jpg}}
    \hfill
  \subfloat[RNN-MBP* \cite{Mao_2022_a}]{%
        \includegraphics[width=0.14\linewidth]{pics/face/face_MBP.jpg}}
    \hfill
  \subfloat[RVRT* \cite{liang2022rvrt}]{%
      \includegraphics[width=0.14\linewidth]{pics/face/face_RVRT.jpg}}
    \hfill
  \subfloat[VRT* \cite{Jin_2021_a}]{%
      \includegraphics[width=0.14\linewidth]{pics/face/face_VRT.jpg}}
    \hfill
  \subfloat[ESTRNN* \cite{zhong2022real}]{%
      \includegraphics[width=0.14\linewidth]{pics/face/face_ESTRNN.jpg}}
    \hfill
  \caption{Qualitative comparison on a dynamic scene sample from the BRIAR dataset \cite{cornett2023expanding}. Figures on the top row are the original restoration results of corresponding TM methods. Figures on the bottom row are models (marked by *) trained on \emph{ATSyn-dynamic} dataset.}
  \label{fig:briar} 
\end{figure*}
Given the impracticality of directly obtaining ground truth images for real-world turbulence scenarios, quantitative performance evaluation typically involves applying restored images to downstream tasks, as noted in \cite{Mao_2022_a, Jaiswal_2023_ICCV, nair2023ddpm}. Adopting this approach, we evaluated various restoration methods using the turbulence text dataset. The results are presented in Fig. \ref{fig:quant_text}, revealing two key insights: 1) our proposed ATSyn-static dataset enhances the generalization capabilities of other TM methods. 2) on both synthetic and real-world sequences, DATUM consistently outperforms other models trained on our dataset. To further validate the effectiveness of our modifications to the Zernike-based simulator, we extensively compared DATUM trained on our ATSyn-dynamic dataset and TMT's dataset \cite{Zhang_2022_a}. We first enhance the long-range subset in the BRIAR dataset \cite{cornett2023expanding} by those two versions, run the same pre-trained face recognition model \cite{Kim_2022_CVPR} on the enhanced images, and it yields the result provided in Table \ref{tab:face}. We can observe the ATSyn-dynamic dataset improved network performance on real-world videos compared to the \cite{Zhang_2022_a} dataset. These comparisons demonstrate our method facilitates better generalization of both scene types than other existing datasets.

We also provide a qualitative comparison in Fig. \ref{fig:text} and \ref{fig:briar} to demonstrate the advance of our network and dataset. By comparing the same networks trained by our data and their original checkpoints, our data enhances their generalization capability. On the other hand, by comparison among all networks trained on our dataset, our model significantly outperforms other networks.
